PromptCap: Prompt-Guided Task-Aware Image Captioning

Knowledge-based visual question answering (VQA) involves questions that require world knowledge beyond the image to yield the correct answer. Large language models (LMs) like GPT-3 are particularly helpful for this task because of their strong knowledge retrieval and reasoning capabilities. To enable LM to understand images, prior work uses a captioning model to convert images into text. However, when summarizing an image in a single caption sentence, which visual entities to describe are often underspecified. Generic image captions often miss visual details essential for the LM to answer visual questions correctly. To address this challenge, we propose PromptCap (Prompt-guided image Captioning), a captioning model designed to serve as a better connector between images and black-box LMs. Different from generic captions, PromptCap takes a natural-language prompt to control the visual entities to describe in the generated caption. The prompt contains a question that the caption should aid in answering. To avoid extra annotation, PromptCap is trained by examples synthesized with GPT-3 and existing datasets. We demonstrate PromptCap's effectiveness on an existing pipeline in which GPT-3 is prompted with image captions to carry out VQA. PromptCap outperforms generic captions by a large margin and achieves state-of-the-art accuracy on knowledge-based VQA tasks (60.4% on OK-VQA and 59.6% on A-OKVQA). Zero-shot results on WebQA show that PromptCap generalizes well to unseen domains.

==> tables/icl.tex <==
\begin{table*}[h]
\small
\centering
\caption{In-context learning results on VQAv2, TextVQA, and OK-VQA. 
Both our systems and Flamingo~\cite{alayrac2022flamingo} uses $n=32$ examples in the prompt.
Frozen \cite{tsimpoukelli2021multimodal} uses $n=4$ examples.
The upper part shows the state of the art by supervised/fine-tuned methods.
%\nascomment{maybe label these with how many labeled examples they each use?}\yushi{we used synthesized data from these datasets to train, so maybe it's better not to bring that up}
}
% \begin{tabular}{P{1.7cm}P{1.2cm}P{1.2cm}P{1.0cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.1cm}P{1.1cm}P{1.1cm}}
\begin{tabular}{lccccccc}
\toprule[1.2pt]
Method & In-Context & Image & \multicolumn{2}{c}{VQAv2} & \multicolumn{2}{c}{TextVQA} & OK-VQA\\
& Example Retrieval & Representation & test-dev & test-std & val & test & val \\
\midrule
\multicolumn{8}{l}{\textbf{Fine-tuned E2E}} \\
%Oscar  &  Feature  & 73.6 & 73.8 \\
%VinVL  & Feature & 75.5 & 75.6 \\
OFA-large \cite{wang2022ofa} & - & Feature  & 80.3 & 80.5 & -& -&-\\
KAT \cite{gui2022kat} & - & Caption + Tags + Feature & - & -& -&- & 54.4\\
GIT \cite{wang2022git} & - & Feature & 78.6 & 78.8 & 59.9 & 59.8 & - \\
%Florence & Feature & 80.2 & 80.4 \\
\midrule
\multicolumn{8}{l}{\textbf{In-Context Learning}} \\
Frozen\cite{tsimpoukelli2021multimodal}  & Random & Feature &  38.2 & - & -  & - & 12.6 \\
Flamingo (80B)\cite{alayrac2022flamingo} & Random & Feature & 67.6 & - & 37.9 & - & 57.8 \\
OFA Cap + GPT-3 & Random & Caption & 61.2 & - & 16.5 & -  & 51.2\\
$\ \ $ + Example Selection & CLIP & Caption & 64.9 & - & 22.6 & - & 55.4 \\
PromptCap + GPT-3 & Random & Caption & 72.1 & - & 48.9 & - & 55.3\\
$\ \ $ + Example Selection & CLIP & Caption & \textbf{74.1} & \textbf{74.1} & \textbf{50.9} & \textbf{51.8} & \textbf{
58.8}\\
% GT + GPT-3 & GT-Caption-5 &  59.7 \\
\bottomrule[1.2pt]

\end{tabular}
\label{tab:icl}

% \bottomrule
 \vspace{-3mm}
\end{table*}

==> tables/okvqa-old.tex <==
\begin{table*}[h]
\small
\centering
% \begin{tabular}{P{1.7cm}P{1.2cm}P{1.2cm}P{1.0cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.1cm}P{1.1cm}P{1.1cm}}
\caption{
\label{tab:okvqa}
Results on the OK-VQA validation set and A-OKVQA test set, with the image representation and the knowledge source each method uses.
Here MC is the multiple-choice accuracy, and DA is the VQA direct-answer accuracy.
The upper part contains the methods that do not rely on large language models as knowledge source, while the methods in the lower part do. 
GPT-3 is frozen for all methods. 
KAT~\cite{gui2022kat} and GPV-2~\cite{kamath2022webly} are the state-of-the-art supervised models for OK-VQA and A-OKVQA, respectively.
}
\begin{tabular}{l|c|l|c|cc}
\toprule[1.2pt]
\multirow{2}{*}{Method} & \multirow{2}{*}{Image Representation} & \multirow{2}{*}{Knowledge Source} & OK-VQA & \multicolumn{2}{c}{A-OKVQA}\\
& & & DA & MC  & DA \\
\midrule
%Pythia\cite{jiang2018pythia} & Feature & - & - & 40.1 & 21.9 \\
%MUTAN\cite{marino2019okvqa} & Feature & - & 26.4 & - & -\\
ConceptBERT\cite{garderes2020conceptbert} &  Feature & ConceptNet & 33.7 &- &-\\
KRISP\cite{marino2021krisp} &  Feature & Wikipedia + ConceptNet & 38.4   & 42.2   &  27.1\\
%Vis-DPR\cite{luo2021weakly}  &  Feature  & Google Search  & 39.2 \\
MAVEx\cite{wu2022multi} & Feature & Wikipedia + ConceptNet + Google Search& 39.4 & - & - \\
GPV-2\cite{kamath2022webly} & Feature & \textsc{Web10k} & -   &  \textbf{53.7}   & 40.7 \\
OFA Cap + FID &  Caption  & Wikipedia &  44.9  & 50.2 & 45.0 \\
\textbf{PromptCap + FID}  & Caption  & Wikipedia & \textbf{48.3}  & 53.1 & \textbf{46.1}\\
\midrule
\multicolumn{4}{l}{\textbf{With LLM}}\\
PICa-Full\cite{yang2022empirical} & Caption + Tags &  GPT-3 (175B) & 48.0 & - & -  \\
KAT (ensemble)\cite{gui2022kat} & Caption + Tags + Feature & GPT-3 (175B) + Wikipedia & 54.4 & - & -  \\
Flamingo (80B)\cite{alayrac2022flamingo} & Feature &  Chinchilla (70B) & 57.8 & - & - \\ 
OFA Cap + GPT-3 &   Caption & GPT-3 (175B) & 55.4  & 70.4 & 53.8 \\
\textbf{PromptCap + GPT-3} & Caption  & GPT-3 (175B) & \textbf{58.8} & \textbf{73.2} & \textbf{58.0}\\
\bottomrule[1.2pt]
\end{tabular}

% \bottomrule
 \vspace{-4mm}
\end{table*}

==> tables/textvqa.tex <==
\begin{table}[h]
\small
\centering
% \begin{tabular}{P{1.7cm}P{1.2cm}P{1.2cm}P{1.0cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.1cm}P{1.1cm}P{1.1cm}}
\begin{tabular}{l|c|cc}
\toprule[1.2pt]
Method & Image & \multicolumn{2}{c}{VQA Acc.} \\
& Repr.& val & test \\
\midrule
\multicolumn{4}{l}{\textbf{Finetuned E2E}} \\
GIT & Feature & & 59.7 \\
\midrule
\multicolumn{4}{l}{\textbf{In-Context Learning}} \\
Flamingo &  Feature & 37.9 & - \\
OFA Cap + GPT3 & Caption & 22.6 & 20.8\\
PromptCap + GPT3 & Caption & 50.9 & 51.8\\
% GT + GPT3 & GT-Caption-5 &  59.7 \\
\bottomrule[1.2pt]
\end{tabular}
\caption{
\label{tab:vqa2}
Results on TextVQA. For in-context learning experiments, we use $n=32$ examples in the prompt. w.o. select 48.9
}
% \bottomrule
 \vspace{-3mm}
\end{table}

==> tables/vqa2.tex <==
\begin{table}[h]
\small
\centering
% \begin{tabular}{P{1.7cm}P{1.2cm}P{1.2cm}P{1.0cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.1cm}P{1.1cm}P{1.1cm}}
\begin{tabular}{l|c|cc}
\toprule[1.2pt]
Method & Image & \multicolumn{2}{c}{VQA Acc.} \\
& Repr.& test-dev & test-std \\
\midrule
\multicolumn{4}{l}{\textbf{Finetuned E2E}} \\
Oscar  &  Feature  & 73.6 & 73.8 \\
VinVL  & Feature & 75.5 & 75.6 \\
OFA-large & Feature  & 80.3 & 80.5 \\
Florence & Feature & 80.2 & 80.4 \\
\midrule
\multicolumn{4}{l}{\textbf{In-Context Learning}} \\
% % Frozen  & Feature  &  38.2 \\
Flamingo &  Feature & 67.6 & - \\
OFA Cap + GPT3 & Caption & 64.9 & 65.4  \\
PromptCap + GPT3 & Caption & 74.1 & 74.1\\
% GT + GPT3 & GT-Caption-5 &  59.7 \\
\bottomrule[1.2pt]
\end{tabular}
\caption{
\label{tab:vqa2}
Results on VQA 2.0 test set. For in-context learning experiments, we use $n=32$ examples in the prompt.
}
% \bottomrule
 \vspace{-3mm}
\end{table}
